MAiVAR: Multimodal Audio-Image and Video Action Recognizer

Currently, action recognition is predominately performed on video data as processed by CNNs. We investigate if the representation process of CNNs can also be leveraged for multimodal action recognition by incorporating image-based audio representations of actions in a task. To this end, we propose Multimodal Audio-Image and Video Action Recognizer (MAiVAR), a CNN-based audio-image to video fusion model that accounts for video and audio modalities to achieve superior action recognition performance. MAiVAR extracts meaningful image representations of audio and fuses it with video representation to achieve better performance as compared to both modalities individually on a large-scale action recognition dataset.

==> extra-text.tex <==

\Comment{
%\begin{figure}[t!]
 %   \centering
 %   \begin{subfigure}[b]{0.4\textwidth}
 %        \centering
 %        \includegraphics[width=\textwidth]{images/video-test-train.PNG}
 %   \caption{Video dataset with 101 classes}
 %        \label{fig:y equals x}
 %    \end{subfigure}
 %    \hfill
  %   \begin{subfigure}[b]{0.4\textwidth}
  %       \centering
  %       \includegraphics[width=\textwidth]{images/audio-test-train.png}
    %\caption{Audio dataset with 51 classes}
    %     \label{fig:three sin x}
    % \end{subfigure}
%    \caption{Training and testing data distribution per class. Training samples (blue bars) and test samples (orange bars). x-axis represents action classes and y-axis represents number of samples.}
 %   \label{fig:train-test}
%\end{figure}
}

Herath et al. \cite{HERATH20174} have deﬁned action as “the most elementary human-surrounding
interaction with a meaning”. HAR is the process of labelling the actions performed by
humans within a given sequence of images, where it becomes the classiﬁcation of goals of
a human agent in a series of image frames. Action recognition typically aims to discover
the class of short, segmented, atomic action. Due to their multifaceted nature,
some of these approaches refer to action recognition as plan recognition, goal recognition,
intent recognition, behavior recognition, location estimation, event recognition, action
recognition, and interaction recognition \cite{shaikh2021rgb}. 

==> results.tex <==
\section{Results}\label{aresults}



\comment{
GFLOPS comparison //
parameters comparison  // 
accuracy comparison //
training / test comparison  //
confusion matrix //
}
